Statistical modeling of the gas-liquid interface using geometrical variables: toward a unified description of the disperse and separated phase flows

In this work, we investigate an original strategy in order to derive a statistical modeling of the interface in gas-liquid two-phase flows through geometrical variables. The con- tribution is two-fold. First it participates in the theoretical design of a unified reduced- order model for the description of two regimes: a disperse phase in a carrier fluid and two separated phases. The first idea is to propose a statistical description of the in- terface relying on geometrical properties such as the mean and Gauss curvatures and define a Surface Density Function (SDF). The second main idea consists in using such a formalism in the disperse case, where a clear link is proposed between local statistics of the interface and the statistics on objects, such as the number density function in Williams-Boltzmann equation for droplets. This makes essential the use of topolog- ical invariants in geometry through the Gauss-Bonnet formula and allows to include the works conducted on sprays of spherical droplets. It yields a statistical treatment of populations of non-spherical objects such as ligaments, as long as they are home- omorphic to a sphere. Second, it provides an original angle and algorithm in order to build statistics from DNS data of interfacial flows. From the theoretical approach, we identify a kernel for the spatial averaging of geometrical quantities preserving the topological invariants. Coupled to a new algorithm for the evaluation of curvatures and surface that preserves these invariants, we analyze two sets of DNS results conducted with the ARCHER code from CORIA with and without topological changes and assess the approach.

==> appendice1.tex <==
Using the equations \eqref{eq:ASDF-requirement1}, \eqref{eq:ASDF-requirement2_3}, \eqref{eq:aaverg} and \eqref{eq:paverg} in the spatial-averaged SDF \eqref{eq:ASDF}, we fulfil the three properties discussed above. However, these equations are not simple to interpret and can introduce more complexities and difficulties in modeling the unclosed terms of the GPBE satisfied by the SDF. Therefore, we propose two simplified averaged SDFs, which do not satisfy all the requirements but which can be more simple to use in the modeling and physical interpretation. For the first one, we use the same equation \eqref{eq:ASDF}, \eqref{eq:aaverg} and \eqref{eq:paverg} but the kernel function is defined as follows:
\begin{equation}
w(\xv;\rv)=\begin{cases}
  0 & \text{if  $||\rv||>h$} \\
  \dfrac{1}{\vol_h}, & \text{otherwise}
  \end{cases}
\end{equation}
where $\vol_h$ is the volume of the set point $\{\rv'\in\mathrm{R}^3,\,\, ||\rv'||<h\}$. The averaged SDF in this case can be written simply as follows:
\begin{equation}
\ASDF(t,\xv;\phasevar)=<\dfrac{S_h(t,\xv)}{\vol_h}\delta(\phasevar-\aaverg{\phasevar}(t,\xv))>
\label{eq:ASDF2}
\end{equation}
where $S_h(t,\xv)=\int_{\yv\in\Volh{\xv}}\delta_I(\yv)\dint{3}{\yv}$ is the area of the surface included in the volume space $\Volh{\xv}$, and the averaged interfacial variables are given by:
\begin{equation}
\paverg{\phasevar}(t,\xv)=\dfrac{1}{S_h(t,\xv)}\int_{\yv\in\Volh{\xv}}\delta_I(\yv)\phasevar(\yv)\dint{3}{\yv}
\end{equation}
The SDF given in \eqref{eq:ASDF2} does not satisfy the first requirement \ref{item:requirement1}, and the second requirement \ref{item:requirement2} can be interpreted in another way, which we will discuss later. The second average SDF, which we propose, reads:
\begin{equation}
\ASDF(t,\xv;\phasevar)=<\delta_I(\xv)\delta(\phasevar-\paverg{\phasevar}(t,\xv))>
\label{eq:ASDF3}
\end{equation}
this time only the interfacial quantities have been spatially-averaged and we keep the same area measure as for the general SDF. This basic averaged SDF satisfies the first and the third requirements but it does not satisfy the conservation of topological information in general case (disperse and separated phases), described in \ref{item:requirement2}. In the following, we adopt the first definition, since it provides a consistent definition of the averaged SDF and satisfies the three required properties. However, for future work and especially if we would to interest to close the equations, it can be more convenient to use one the two last simplified averaged SDF. In the results section, we will compare the two last SDF and we will give an other interpretation of the third requirement in the case of the averaged SDF given in \eqref{eq:ASDF2}.

